Forecasting Probability of Default for Consumer Loan Management with Gaussian Mixture Models

Credit scoring is an essential tool used by global financial institutions and credit lenders for financial decision making. In this paper, we introduce a new method based on Gaussian Mixture Model (GMM) to forecast the probability of default for individual loan applicants. Clustering similar customers with each other, our model associates a probability of being healthy to each group. In addition, our GMM-based model probabilistically associates individual samples to clusters, and then estimates the probability of default for each individual based on how it relates to GMM clusters. We provide applications for risk managers and decision makers in banks and non-bank financial institutions to maximize profit and mitigate the expected loss by giving loans to those who have a probability of default below a decision threshold. Our model has a number of advantages. First, it gives a probabilistic view of credit standing for each individual applicant instead of a binary classification and therefore provides more information for financial decision makers. Second, the expected loss on the train set calculated by our GMM-based default probabilities is very close to the actual loss, and third, our approach is computationally efficient.

==> figs/LaTeX_figs/barplot_test.tex <==
\begin{tikzpicture}
\pgfmathsetmacro{\radius}{20}
\pgfmathsetmacro{\graphicshift}{0}
\pgfmathsetmacro{\legendshift}{-30}

\definecolor{colorChebychev}{HTML}{55c968}

%\definecolor{colorEuclidean}{HTML}{800000}
\definecolor{colorEuclidean}{HTML}{DE4040}

%\definecolor{colorManhattan}{HTML}{FF0000}
\definecolor{colorManhattan}{HTML}{5872bf}

%\definecolor{colorCamberra}{HTML}{FF8000}
\definecolor{colorCamberra}{HTML}{2793DA}


\definecolor{colorMinkowsky}{HTML}{FFFF00}

\colorlet{colorLines}{gray!50!white}
\colorlet{colorMainLines}{gray}

\tikzset{colorEuclidean40/.style={fill=colorEuclidean,draw=black}}
\tikzset{colorManhattan40/.style={fill=colorManhattan,draw=black}}
\tikzset{colorCamberra40/.style={fill=colorCamberra,draw=black}}
\tikzset{colorChebychev40/.style={fill=colorChebychev,draw=black}}
\tikzset{colorMinkowsky40/.style={fill=colorMinkowsky,draw=black}}

\tikzset{colorEuclidean20/.style={draw=black,line width=0.1cm}}
\tikzset{colorManhattan20/.style={draw=black,line width=0.1cm}}
\tikzset{colorCamberra20/.style= {draw=black,line width=0.1cm}}
\tikzset{colorChebychev20/.style={draw=black,line width=0.1cm}}
\tikzset{colorMinkowsky20/.style={draw=black,line width=0.1cm}}

\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorCamberra40] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		}};
	
% 10º arches		
\foreach \a in {0, ..., 5} {
	\foreach \m in {0, ..., 16} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 10: 1.3* \radius);
		}};		
	
\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		};
\draw[colorMainLines] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
	\draw[colorMainLines, yshift=\graphicshift cm] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
};

% Concentric Circles
\foreach \p in {0.5,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9, 0.95,1.0, 1.475, 1.3, 1.6} {
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorLines] (0,0) circle (\r);
	\draw[colorLines, yshift=\graphicshift cm] (0,0) circle (\r);	
};

\foreach \p in {1} {
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorCamberra20] (0,0) circle (\r);
	\draw[colorCamberra20, yshift=\graphicshift cm] (0,0) circle (\r);	
};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metrics - Australian Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (75:\r) {\Huge{\textbf{AUC score}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (45:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-75] at (15:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-105] at (-15:\r) {\Huge{\textbf{$F_1$ score}}};

\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=-60] at (30:\r) {\Huge{\textbf{Australian}}};

% Metrics - Japanese Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+25+40+40+40+40+40:\r) {\Huge{\textbf{AUC score}}};


\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+25+10+40+40+40+40:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (90+20-15+40+40+40+40:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (90+20-15+40+40+40+40-30:\r) {\Huge{\textbf{$F_1$ score}}};


\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=0] at (30-120:\r) {\Huge{\textbf{Japanese}}};


% Metrics - German Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+15:\r) {\Huge{\textbf{$F_1$ score}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+15+30:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=75] at (90+15+30+30:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=105] at (90+15+30+30+30:\r) {\Huge{\textbf{AUC score}}};


\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=60] at (30-120*2:\r) {\Huge{\textbf{German}}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Australian
% AUC score Australian
\pgfmathsetmacro{\r}{0.7862*\radius} 
\draw[colorChebychev40](90:\r)--(0,0)--(90-10*1:\r) arc (90-10*1:90:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*1] at (90-5*1:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7862}$}};

\pgfmathsetmacro{\r}{0.6991*\radius} 
\draw[colorEuclidean40](90-10*1:\r)--(0,0)--(90-10*2:\r) arc (90-10*2:90-10*1:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*3] at (90-5*3:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6991}$}};

\pgfmathsetmacro{\r}{0.8823*\radius} 
\draw[colorManhattan40](90-10*2:\r)--(0,0)--(90-10*3:\r) arc (90-10*3:90-10*2:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*5] at (90-5*5:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8823}$}};

% Precision Australian

\pgfmathsetmacro{\r}{0.8395*\radius} 
\draw[colorChebychev40](90-10*3:\r)--(0,0)--(90-10*4:\r) arc (90-10*4:90-10*3:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*7] at (90-5*7:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8395}$}};

\pgfmathsetmacro{\r}{0.7674*\radius} %dois
\draw[colorEuclidean40](90-10*4:\r)--(0,0)--(90-10*5:\r) arc (90-10*5:90-10*4:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*9] at (90-5*9:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7674}$}};

\pgfmathsetmacro{\r}{0.8470*\radius} %dois
\draw[colorManhattan40](90-10*5:\r)--(0,0)--(90-10*6:\r) arc (90-10*6:90-10*5:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*11] at (90-5*11:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8470}$}};

% Recall Australian


\pgfmathsetmacro{\r}{0.6732*\radius} %dois
\draw[colorChebychev40](90-10*6:\r)--(0,0)--(90-10*7:\r) arc (90-10*7:90-10*6:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*13] at (90-5*13:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6732}$}};

\pgfmathsetmacro{\r}{0.3267*\radius} %dois
\draw[colorEuclidean40](90-10*7:\r)--(0,0)--(90-10*8:\r) arc (90-10*8:90-10*7:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*15] at (90-5*15:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3267}$}};

\pgfmathsetmacro{\r}{0.7128*\radius} %dois
\draw[colorManhattan40](90-10*8:\r)--(0,0)--(90-10*9:\r) arc (90-10*9:90-10*8:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*17] at (90-5*17:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7128}$}};
% $F_1$ score Australian
\pgfmathsetmacro{\r}{0.7472*\radius} 
\draw[colorChebychev40](90-10*9:\r)--(0,0)--(90-10*10:\r) arc (90-10*10:90-10*9:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*19] at (90-5*19:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7472}$}};

\pgfmathsetmacro{\r}{0.4583*\radius} 
\draw[colorEuclidean40](90-10*10:\r)--(0,0)--(90-10*11:\r) arc (90-10*11:90-10*10:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*21] at (90-5*21:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4583}$}};

\pgfmathsetmacro{\r}{0.7741*\radius} 
\draw[colorManhattan40](90-10*11:\r)--(0,0)--(90-10*12:\r) arc (90-10*12:90-10*11:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*23] at (90-5*23:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7741}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sampling Japanese

% AUC score Japanese

\pgfmathsetmacro{\r}{0.8340*\radius} 
\draw[colorChebychev40](90-10*12:\r)--(0,0)--(90-10*13:\r) arc (90-10*13:90-10*12:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*25] at (90-5*25:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8340}$}};

\pgfmathsetmacro{\r}{0.7321*\radius} 
\draw[colorEuclidean40](90-10*13:\r)--(0,0)--(90-10*14:\r) arc (90-10*14:90-10*13:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*27] at (90-5*27:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7321}$}};

\pgfmathsetmacro{\r}{0.8692*\radius} 
\draw[colorManhattan40](90-10*14:\r)--(0,0)--(90-10*15:\r) arc (90-10*15:90-10*14:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*29] at (90-5*29:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8692}$}};
% Precision Japanese

\pgfmathsetmacro{\r}{0.8181*\radius} 
\draw[colorChebychev40](90-10*15:\r)--(0,0)--(90-10*16:\r) arc (90-10*16:90-10*15:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*31] at (90-5*31:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8181}$}};

\pgfmathsetmacro{\r}{0.7391*\radius} 
\draw[colorEuclidean40](90-10*16:\r)--(0,0)--(90-10*17:\r) arc (90-10*17:90-10*16:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*33] at (90-5*33:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7391}$}};

\pgfmathsetmacro{\r}{0.8043*\radius} 
\draw[colorManhattan40](90-10*17:\r)--(0,0)--(90-10*18:\r) arc (90-10*18:90-10*17:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*35] at (90-5*35:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8043}$}};
% Recall Japanese

\pgfmathsetmacro{\r}{0.7912*\radius} 
\draw[colorChebychev40](90-10*18:\r)--(0,0)--(90-10*19:\r) arc (90-10*19:90-10*18:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*37+180] at (90-5*37:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7912}$}};

\pgfmathsetmacro{\r}{0.3736*\radius} 
\draw[colorEuclidean40](90-10*19:\r)--(0,0)--(90-10*20:\r) arc (90-10*20:90-10*19:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*39+180] at (90-5*39:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3736}$}};

\pgfmathsetmacro{\r}{0.8131*\radius} 
\draw[colorManhattan40](90-10*20:\r)--(0,0)--(90-10*21:\r) arc (90-10*21:90-10*20:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*41+180] at (90-5*41:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8131}$}};
% $F_1$ score Japanese

\pgfmathsetmacro{\r}{0.8044*\radius} 
\draw[colorChebychev40](90-10*21:\r)--(0,0)--(90-10*22:\r) arc (90-10*22:90-10*21:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*43+180] at (90-5*43:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8044}$}};

\pgfmathsetmacro{\r}{0.4963*\radius} 
\draw[colorEuclidean40](90-10*22:\r)--(0,0)--(90-10*23:\r) arc (90-10*23:90-10*22:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*45+180] at (90-5*45:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4963}$}};

\pgfmathsetmacro{\r}{0.8087*\radius} 
\draw[colorManhattan40](90-10*23:\r)--(0,0)--(90-10*24:\r) arc (90-10*24:90-10*23:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*47+180] at (90-5*47:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8087}$}};

% German

% AUC score German
\pgfmathsetmacro{\r}{0.4979*\radius} 
\draw[colorChebychev40](90-10*24:\r)--(0,0)--(90-10*25:\r) arc (90-10*25:90-10*24:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*49+180] at (90-5*49:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4979}$}};

\pgfmathsetmacro{\r}{0.5859*\radius} 
\draw[colorEuclidean40](90-10*25:\r)--(0,0)--(90-10*26:\r) arc (90-10*26:90-10*25:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*51+180] at (90-5*51:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.5859}$ }};


\pgfmathsetmacro{\r}{0.7696*\radius} 
\draw[colorManhattan40](90-10*26:\r)--(0,0)--(90-10*27:\r) arc (90-10*27:90-10*26:\r);
\pgfmathsetmacro{\r}{\radius + 3} 
\node[rotate=90-5*53+180] at (90-5*53:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7696}$}};

% Precision German
\pgfmathsetmacro{\r}{0.7237*\radius} 
\draw[colorChebychev40](90-10*27:\r)--(0,0)--(90-10*28:\r) arc (90-10*28:90-10*27:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*55+180] at (90-5*55:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7237}$}};


\pgfmathsetmacro{\r}{0.7568*\radius} 
\draw[colorEuclidean40](90-10*28:\r)--(0,0)--(90-10*29:\r) arc (90-10*29:90-10*28:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*57+180] at (90-5*57:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7568}$}};

\pgfmathsetmacro{\r}{0.8163*\radius} 
\draw[colorManhattan40](90-10*29:\r)--(0,0)--(90-10*30:\r) arc (90-10*30:90-10*29:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*59+180] at (90-5*59:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8163}$}};

% Recall score German

\pgfmathsetmacro{\r}{0.9958*\radius} 
\draw[colorChebychev40](90-10*30:\r)--(0,0)--(90-10*31:\r) arc (90-10*31:90-10*30:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*61+180] at (90-5*61:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.9958}$}};

\pgfmathsetmacro{\r}{0.7975*\radius} 
\draw[colorEuclidean40](90-10*31:\r)--(0,0)--(90-10*32:\r) arc (90-10*32:90-10*31:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*63+180] at (90-5*63:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7975}$}};

\pgfmathsetmacro{\r}{0.8264*\radius} 
\draw[colorManhattan40](90-10*32:\r)--(0,0)--(90-10*33:\r) arc (90-10*33:90-10*32:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*65+180] at (90-5*65:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8264}$}};


% $F_1$ score German

\pgfmathsetmacro{\r}{0.8382*\radius} 
\draw[colorChebychev40](90-10*33:\r)--(0,0)--(90-10*34:\r) arc (90-10*34:90-10*33:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*67+180] at (90-5*67:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8382}$}};

\pgfmathsetmacro{\r}{0.7766*\radius} 
\draw[colorEuclidean40](90-10*34:\r)--(0,0)--(90-10*35:\r) arc (90-10*35:90-10*34:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*69+180] at (90-5*69:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7766}$}};
    
\pgfmathsetmacro{\r}{0.8213*\radius} 
\draw[colorManhattan40](90-10*35:\r)--(0,0)--(90-10*36:\r) arc (90-10*36:90-10*35:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*71+180] at (90-5*71:\r) {\scalebox{1.175}[1.0]{\huge$\mathbf{0.8213}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 'Mercedes symbol' bold
\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorCamberra20] (0, 0) -- (90 - \a * 120 - \m * 120 : 1.6* \radius);
		}};
		
	
% Other bolds		

\foreach \m in {0, ..., 12}{
\draw[colorCamberra20] (0, 0) -- (90 - \m * 30 : 1.475* \radius);
};			
			
 Center
\draw[colorCamberra20, fill=white] (0,0) circle (0.2 * \radius);
\node at (0,0) {\Huge test data};
\draw[colorCamberra20, fill=white, yshift=\graphicshift cm] (0,0) circle (0.2 * \radius);
\node at (0,\graphicshift+0.5 cm){\Huge\textbf{Test Set}};
\node at (0,\graphicshift-0.5 cm){\Huge\textbf{}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Caption
\coordinate (rc) at (-20cm,-6cm \legendshift cm);
\foreach \m/\c in {GMM/colorChebychev,SVM/colorEuclidean,LR/colorManhattan} {
	\node[right of=rc, node distance=8cm, rectangle, draw=colorMainLines, fill=\c, minimum width=1.5cm, minimum height=0.825cm] (rc) {};
	\node[right of=rc, node distance=0.8cm, anchor=west] {\Huge \m};
}
\end{tikzpicture}
% \label{fig:M1}




==> figs/LaTeX_figs/barplot_train.tex <==
\begin{tikzpicture}
% \label{fig:M1}
\pgfmathsetmacro{\radius}{20}
\pgfmathsetmacro{\graphicshift}{0}
\pgfmathsetmacro{\legendshift}{-30}

\definecolor{colorChebychev}{HTML}{55c968}

%\definecolor{colorEuclidean}{HTML}{800000}
\definecolor{colorEuclidean}{HTML}{DE4040}

%\definecolor{colorManhattan}{HTML}{FF0000}
\definecolor{colorManhattan}{HTML}{5872bf}

%\definecolor{colorCamberra}{HTML}{FF8000}
\definecolor{colorCamberra}{HTML}{2793DA}


\definecolor{colorMinkowsky}{HTML}{FFFF00}

\colorlet{colorLines}{gray!50!white}
\colorlet{colorMainLines}{gray}

\tikzset{colorEuclidean40/.style={fill=colorEuclidean,draw=black}}
\tikzset{colorManhattan40/.style={fill=colorManhattan,draw=black}}
\tikzset{colorCamberra40/.style={fill=colorCamberra,draw=black}}
\tikzset{colorChebychev40/.style={fill=colorChebychev,draw=black}}
\tikzset{colorMinkowsky40/.style={fill=colorMinkowsky,draw=black}}

\tikzset{colorEuclidean20/.style={draw=black,line width=0.1cm}}
\tikzset{colorManhattan20/.style={draw=black,line width=0.1cm}}
\tikzset{colorCamberra20/.style= {draw=black,line width=0.1cm}}
\tikzset{colorChebychev20/.style={draw=black,line width=0.1cm}}
\tikzset{colorMinkowsky20/.style={draw=black,line width=0.1cm}}

\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorCamberra40] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		}};
	
% 10º arches		
\foreach \a in {0, ..., 5} {
	\foreach \m in {0, ..., 16} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 10: 1.3* \radius);
		}};		
	
\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		};
\draw[colorMainLines] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
	\draw[colorMainLines, yshift=\graphicshift cm] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
};

% Concentric Circles
\foreach \p in {0.5,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9, 0.95,1.0, 1.475, 1.3, 1.6} {
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorLines] (0,0) circle (\r);
	\draw[colorLines, yshift=\graphicshift cm] (0,0) circle (\r);	
};

\foreach \p in {1} {
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorCamberra20] (0,0) circle (\r);
	\draw[colorCamberra20, yshift=\graphicshift cm] (0,0) circle (\r);	
};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metrics - Australian Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (75:\r) {\Huge{\textbf{AUC score}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (45:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-75] at (15:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-105] at (-15:\r) {\Huge{\textbf{$F_1$ score}}};

\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=-60] at (30:\r) {\Huge{\textbf{Australian}}};

% Metrics - Japanese Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+25+40+40+40+40+40:\r) {\Huge{\textbf{AUC score}}};


\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+25+10+40+40+40+40:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (90+20-15+40+40+40+40:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (90+20-15+40+40+40+40-30:\r) {\Huge{\textbf{$F_1$ score}}};


\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=0] at (30-120:\r) {\Huge{\textbf{Japanese}}};


% Metrics - German Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+15:\r) {\Huge{\textbf{$F_1$ score}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+15+30:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=75] at (90+15+30+30:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=105] at (90+15+30+30+30:\r) {\Huge{\textbf{AUC score}}};


\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=60] at (30-120*2:\r) {\Huge{\textbf{German}}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Australian
% AUC score Australian
\pgfmathsetmacro{\r}{0.8134*\radius} 
\draw[colorChebychev40](90:\r)--(0,0)--(90-10*1:\r) arc (90-10*1:90:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*1] at (90-5*1:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8134}$}};

\pgfmathsetmacro{\r}{0.6983*\radius} 
\draw[colorEuclidean40](90-10*1:\r)--(0,0)--(90-10*2:\r) arc (90-10*2:90-10*1:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*3] at (90-5*3:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6983}$}};

\pgfmathsetmacro{\r}{0.9157*\radius} 
\draw[colorManhattan40](90-10*2:\r)--(0,0)--(90-10*3:\r) arc (90-10*3:90-10*2:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*5] at (90-5*5:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.9157}$}};

% Precision Australian

\pgfmathsetmacro{\r}{0.8698*\radius} 
\draw[colorChebychev40](90-10*3:\r)--(0,0)--(90-10*4:\r) arc (90-10*4:90-10*3:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*7] at (90-5*7:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8698}$}};

\pgfmathsetmacro{\r}{0.7954*\radius} %dois
\draw[colorEuclidean40](90-10*4:\r)--(0,0)--(90-10*5:\r) arc (90-10*5:90-10*4:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*9] at (90-5*9:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7954}$}};

\pgfmathsetmacro{\r}{0.8688*\radius} %dois
\draw[colorManhattan40](90-10*5:\r)--(0,0)--(90-10*6:\r) arc (90-10*6:90-10*5:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*11] at (90-5*11:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8688}$}};

% Recall Australian


\pgfmathsetmacro{\r}{0.7135*\radius} %dois
\draw[colorChebychev40](90-10*6:\r)--(0,0)--(90-10*7:\r) arc (90-10*7:90-10*6:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*13] at (90-5*13:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7135}$}};

\pgfmathsetmacro{\r}{0.3398*\radius} %dois
\draw[colorEuclidean40](90-10*7:\r)--(0,0)--(90-10*8:\r) arc (90-10*8:90-10*7:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*15] at (90-5*15:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3398}$}};

\pgfmathsetmacro{\r}{0.7718*\radius} %dois
\draw[colorManhattan40](90-10*8:\r)--(0,0)--(90-10*9:\r) arc (90-10*9:90-10*8:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*17] at (90-5*17:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7718}$}};
% $F_1$ score Australian
\pgfmathsetmacro{\r}{0.7839*\radius} 
\draw[colorChebychev40](90-10*9:\r)--(0,0)--(90-10*10:\r) arc (90-10*10:90-10*9:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*19] at (90-5*19:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7839}$}};

\pgfmathsetmacro{\r}{0.4761*\radius} 
\draw[colorEuclidean40](90-10*10:\r)--(0,0)--(90-10*11:\r) arc (90-10*11:90-10*10:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*21] at (90-5*21:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4761}$}};

\pgfmathsetmacro{\r}{0.8174*\radius} 
\draw[colorManhattan40](90-10*11:\r)--(0,0)--(90-10*12:\r) arc (90-10*12:90-10*11:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*23] at (90-5*23:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8174}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sampling Japanese

% AUC score Japanese

\pgfmathsetmacro{\r}{0.8399*\radius} 
\draw[colorChebychev40](90-10*12:\r)--(0,0)--(90-10*13:\r) arc (90-10*13:90-10*12:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*25] at (90-5*25:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8399}$}};

\pgfmathsetmacro{\r}{0.6931*\radius} 
\draw[colorEuclidean40](90-10*13:\r)--(0,0)--(90-10*14:\r) arc (90-10*14:90-10*13:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*27] at (90-5*27:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6931}$}};

\pgfmathsetmacro{\r}{0.8967*\radius} 
\draw[colorManhattan40](90-10*14:\r)--(0,0)--(90-10*15:\r) arc (90-10*15:90-10*14:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*29] at (90-5*29:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8967}$}};
% Precision Japanese

\pgfmathsetmacro{\r}{0.8702*\radius} 
\draw[colorChebychev40](90-10*15:\r)--(0,0)--(90-10*16:\r) arc (90-10*16:90-10*15:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*31] at (90-5*31:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8702}$}};

\pgfmathsetmacro{\r}{0.8235*\radius} 
\draw[colorEuclidean40](90-10*16:\r)--(0,0)--(90-10*17:\r) arc (90-10*17:90-10*16:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*33] at (90-5*33:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8235}$}};

\pgfmathsetmacro{\r}{0.8241*\radius} 
\draw[colorManhattan40](90-10*17:\r)--(0,0)--(90-10*18:\r) arc (90-10*18:90-10*17:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*35] at (90-5*35:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8241}$}};
% Recall Japanese

\pgfmathsetmacro{\r}{0.7815*\radius} 
\draw[colorChebychev40](90-10*18:\r)--(0,0)--(90-10*19:\r) arc (90-10*19:90-10*18:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*37+180] at (90-5*37:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7815}$}};

\pgfmathsetmacro{\r}{0.3398*\radius} 
\draw[colorEuclidean40](90-10*19:\r)--(0,0)--(90-10*20:\r) arc (90-10*20:90-10*19:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*39+180] at (90-5*39:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3398}$}};

\pgfmathsetmacro{\r}{0.7961*\radius} 
\draw[colorManhattan40](90-10*20:\r)--(0,0)--(90-10*21:\r) arc (90-10*21:90-10*20:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*41+180] at (90-5*41:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7961}$}};
% $F_1$ score Japanese

\pgfmathsetmacro{\r}{0.8235*\radius} 
\draw[colorChebychev40](90-10*21:\r)--(0,0)--(90-10*22:\r) arc (90-10*22:90-10*21:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*43+180] at (90-5*43:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8235}$}};

\pgfmathsetmacro{\r}{0.4810*\radius} 
\draw[colorEuclidean40](90-10*22:\r)--(0,0)--(90-10*23:\r) arc (90-10*23:90-10*22:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*45+180] at (90-5*45:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4810}$}};

\pgfmathsetmacro{\r}{0.8980*\radius} 
\draw[colorManhattan40](90-10*23:\r)--(0,0)--(90-10*24:\r) arc (90-10*24:90-10*23:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*47+180] at (90-5*47:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8980}$}};

% German

% AUC score German
\pgfmathsetmacro{\r}{0.7423*\radius} 
\draw[colorChebychev40](90-10*24:\r)--(0,0)--(90-10*25:\r) arc (90-10*25:90-10*24:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*49+180] at (90-5*49:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7423}$}};

\pgfmathsetmacro{\r}{0.5623*\radius} 
\draw[colorEuclidean40](90-10*25:\r)--(0,0)--(90-10*26:\r) arc (90-10*26:90-10*25:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*51+180] at (90-5*51:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.5623}$ }};


\pgfmathsetmacro{\r}{0.8945*\radius} 
\draw[colorManhattan40](90-10*26:\r)--(0,0)--(90-10*27:\r) arc (90-10*27:90-10*26:\r);
\pgfmathsetmacro{\r}{\radius + 3} 
\node[rotate=90-5*53+180] at (90-5*53:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8945}$}};

% Precision German
\pgfmathsetmacro{\r}{0.6767*\radius} 
\draw[colorChebychev40](90-10*27:\r)--(0,0)--(90-10*28:\r) arc (90-10*28:90-10*27:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*55+180] at (90-5*55:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6767}$}};


\pgfmathsetmacro{\r}{0.5306*\radius} 
\draw[colorEuclidean40](90-10*28:\r)--(0,0)--(90-10*29:\r) arc (90-10*29:90-10*28:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*57+180] at (90-5*57:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.5306}$}};

\pgfmathsetmacro{\r}{0.8245*\radius} 
\draw[colorManhattan40](90-10*29:\r)--(0,0)--(90-10*30:\r) arc (90-10*30:90-10*29:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*59+180] at (90-5*59:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8245}$}};

% Recall score German

\pgfmathsetmacro{\r}{0.9279*\radius} 
\draw[colorChebychev40](90-10*30:\r)--(0,0)--(90-10*31:\r) arc (90-10*31:90-10*30:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*61+180] at (90-5*61:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.9279}$}};

\pgfmathsetmacro{\r}{0.8318*\radius} 
\draw[colorEuclidean40](90-10*31:\r)--(0,0)--(90-10*32:\r) arc (90-10*32:90-10*31:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*63+180] at (90-5*63:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8318}$}};

\pgfmathsetmacro{\r}{0.8209*\radius} 
\draw[colorManhattan40](90-10*32:\r)--(0,0)--(90-10*33:\r) arc (90-10*33:90-10*32:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*65+180] at (90-5*65:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8209}$}};


% $F_1$ score German

\pgfmathsetmacro{\r}{0.7826*\radius} 
\draw[colorChebychev40](90-10*33:\r)--(0,0)--(90-10*34:\r) arc (90-10*34:90-10*33:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*67+180] at (90-5*67:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7826}$}};

\pgfmathsetmacro{\r}{0.6479*\radius} 
\draw[colorEuclidean40](90-10*34:\r)--(0,0)--(90-10*35:\r) arc (90-10*35:90-10*34:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*69+180] at (90-5*69:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6479}$}};
    
\pgfmathsetmacro{\r}{0.8227*\radius} 
\draw[colorManhattan40](90-10*35:\r)--(0,0)--(90-10*36:\r) arc (90-10*36:90-10*35:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*71+180] at (90-5*71:\r) {\scalebox{1.175}[1.0]{\huge$\mathbf{0.8227}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 'Mercedes symbol' bold
\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorCamberra20] (0, 0) -- (90 - \a * 120 - \m * 120 : 1.6* \radius);
		}};
% Other bolds
\foreach \m in {0, ..., 12}{
\draw[colorCamberra20] (0, 0) -- (90 - \m * 30 : 1.475* \radius);
};			
			
 Center
\draw[colorCamberra20, fill=white] (0,0) circle (0.2 * \radius);
\node at (0,0) {\Huge Train data};
\draw[colorCamberra20, fill=white, yshift=\graphicshift cm] (0,0) circle (0.2 * \radius);
\node at (0,\graphicshift+0.5 cm){\Huge\textbf{Train Set}};
\node at (0,\graphicshift-0.5 cm){\Huge\textbf{}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Caption
\coordinate (rc) at (-20cm,-6cm \legendshift cm);
\foreach \m/\c in {GMM/colorChebychev,SVM/colorEuclidean,LR/colorManhattan} {
	\node[right of=rc, node distance=8cm, rectangle, draw=colorMainLines, fill=\c, minimum width=1.5cm, minimum height=0.825cm] (rc) {};
	\node[right of=rc, node distance=0.8cm, anchor=west] {\Huge \m};
}
\end{tikzpicture}

==> figs/LaTeX_figs/cobweb2.tex <==
% %% 
% %% Copyright 2007, 2008, 2009 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% %% ---------------------------------------------
% %% 
% %% It may be distributed under the conditions of the LaTeX Project Public
% %% Author: Francisco Antunes

\begin{figure*}
	\begin{center}
	\resizebox{5in}{5in}{
			\begin{tikzpicture}
\pgfmathsetmacro{\radius}{20}
\pgfmathsetmacro{\graphicshift}{0}
\pgfmathsetmacro{\legendshift}{-30}

\definecolor{colorChebychev}{HTML}{55c968}

%\definecolor{colorEuclidean}{HTML}{800000}
\definecolor{colorEuclidean}{HTML}{DE4040}

%\definecolor{colorManhattan}{HTML}{FF0000}
\definecolor{colorManhattan}{HTML}{5872bf}

%\definecolor{colorCamberra}{HTML}{FF8000}
\definecolor{colorCamberra}{HTML}{2793DA}


\definecolor{colorMinkowsky}{HTML}{FFFF00}

\colorlet{colorLines}{gray!50!white}
\colorlet{colorMainLines}{gray}

\tikzset{colorEuclidean40/.style={fill=colorEuclidean,draw=black}}
\tikzset{colorManhattan40/.style={fill=colorManhattan,draw=black}}
\tikzset{colorCamberra40/.style={fill=colorCamberra,draw=black}}
\tikzset{colorChebychev40/.style={fill=colorChebychev,draw=black}}
\tikzset{colorMinkowsky40/.style={fill=colorMinkowsky,draw=black}}

\tikzset{colorEuclidean20/.style={draw=black,line width=0.1cm}}
\tikzset{colorManhattan20/.style={draw=black,line width=0.1cm}}
\tikzset{colorCamberra20/.style= {draw=black,line width=0.1cm}}
\tikzset{colorChebychev20/.style={draw=black,line width=0.1cm}}
\tikzset{colorMinkowsky20/.style={draw=black,line width=0.1cm}}

\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorCamberra40] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		}};
	
% 10º arches		
\foreach \a in {0, ..., 5} {
	\foreach \m in {0, ..., 16} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 10: 1.3* \radius);
		}};		
	
\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		};
\draw[colorMainLines] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
	\draw[colorMainLines, yshift=\graphicshift cm] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
};

% Concentric Circles
\foreach \p in {0.5,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9, 0.95,1.0, 1.475, 1.3, 1.6} {
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorLines] (0,0) circle (\r);
	\draw[colorLines, yshift=\graphicshift cm] (0,0) circle (\r);	
};

\foreach \p in {1} {
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorCamberra20] (0,0) circle (\r);
	\draw[colorCamberra20, yshift=\graphicshift cm] (0,0) circle (\r);	
};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metrics - Australian Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (75:\r) {\Huge{\textbf{AUC score}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (45:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-75] at (15:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-105] at (-15:\r) {\Huge{\textbf{$F_1$ score}}};

\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=-60] at (30:\r) {\Huge{\textbf{Australian}}};

% Metrics - Japanese Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+25+40+40+40+40+40:\r) {\Huge{\textbf{AUC score}}};


\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+25+10+40+40+40+40:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (90+20-15+40+40+40+40:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (90+20-15+40+40+40+40-30:\r) {\Huge{\textbf{$F_1$ score}}};


\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=0] at (30-120:\r) {\Huge{\textbf{Japanese}}};


% Metrics - German Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+15:\r) {\Huge{\textbf{$F_1$ score}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+15+30:\r) {\Huge{\textbf{Recall}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=75] at (90+15+30+30:\r) {\Huge{\textbf{Precision}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=105] at (90+15+30+30+30:\r) {\Huge{\textbf{AUC score}}};


\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=60] at (30-120*2:\r) {\Huge{\textbf{German}}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Australian
% AUC score Australian
\pgfmathsetmacro{\r}{0.7862*\radius} 
\draw[colorChebychev40](90:\r)--(0,0)--(90-10*1:\r) arc (90-10*1:90:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*1] at (90-5*1:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7862}$}};

\pgfmathsetmacro{\r}{0.6991*\radius} 
\draw[colorEuclidean40](90-10*1:\r)--(0,0)--(90-10*2:\r) arc (90-10*2:90-10*1:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*3] at (90-5*3:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6991}$}};

\pgfmathsetmacro{\r}{0.8823*\radius} 
\draw[colorManhattan40](90-10*2:\r)--(0,0)--(90-10*3:\r) arc (90-10*3:90-10*2:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*5] at (90-5*5:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8823}$}};

% Precision Australian

\pgfmathsetmacro{\r}{0.8395*\radius} 
\draw[colorChebychev40](90-10*3:\r)--(0,0)--(90-10*4:\r) arc (90-10*4:90-10*3:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*7] at (90-5*7:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8395}$}};

\pgfmathsetmacro{\r}{0.7674*\radius} %dois
\draw[colorEuclidean40](90-10*4:\r)--(0,0)--(90-10*5:\r) arc (90-10*5:90-10*4:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*9] at (90-5*9:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7674}$}};

\pgfmathsetmacro{\r}{0.8470*\radius} %dois
\draw[colorManhattan40](90-10*5:\r)--(0,0)--(90-10*6:\r) arc (90-10*6:90-10*5:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*11] at (90-5*11:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8470}$}};

% Recall Australian


\pgfmathsetmacro{\r}{0.6732*\radius} %dois
\draw[colorChebychev40](90-10*6:\r)--(0,0)--(90-10*7:\r) arc (90-10*7:90-10*6:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*13] at (90-5*13:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6732}$}};

\pgfmathsetmacro{\r}{0.3267*\radius} %dois
\draw[colorEuclidean40](90-10*7:\r)--(0,0)--(90-10*8:\r) arc (90-10*8:90-10*7:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*15] at (90-5*15:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3267}$}};

\pgfmathsetmacro{\r}{0.7128*\radius} %dois
\draw[colorManhattan40](90-10*8:\r)--(0,0)--(90-10*9:\r) arc (90-10*9:90-10*8:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*17] at (90-5*17:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7128}$}};
% $F_1$ score Australian
\pgfmathsetmacro{\r}{0.7472*\radius} 
\draw[colorChebychev40](90-10*9:\r)--(0,0)--(90-10*10:\r) arc (90-10*10:90-10*9:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*19] at (90-5*19:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7472}$}};

\pgfmathsetmacro{\r}{0.4583*\radius} 
\draw[colorEuclidean40](90-10*10:\r)--(0,0)--(90-10*11:\r) arc (90-10*11:90-10*10:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*21] at (90-5*21:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4583}$}};

\pgfmathsetmacro{\r}{0.7741*\radius} 
\draw[colorManhattan40](90-10*11:\r)--(0,0)--(90-10*12:\r) arc (90-10*12:90-10*11:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*23] at (90-5*23:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7741}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sampling Japanese

% AUC score Japanese

\pgfmathsetmacro{\r}{0.8340*\radius} 
\draw[colorChebychev40](90-10*12:\r)--(0,0)--(90-10*13:\r) arc (90-10*13:90-10*12:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*25] at (90-5*25:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8340}$}};

\pgfmathsetmacro{\r}{0.7321*\radius} 
\draw[colorEuclidean40](90-10*13:\r)--(0,0)--(90-10*14:\r) arc (90-10*14:90-10*13:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*27] at (90-5*27:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7321}$}};

\pgfmathsetmacro{\r}{0.8692*\radius} 
\draw[colorManhattan40](90-10*14:\r)--(0,0)--(90-10*15:\r) arc (90-10*15:90-10*14:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*29] at (90-5*29:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8692}$}};
% Precision Japanese

\pgfmathsetmacro{\r}{0.8181*\radius} 
\draw[colorChebychev40](90-10*15:\r)--(0,0)--(90-10*16:\r) arc (90-10*16:90-10*15:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*31] at (90-5*31:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8181}$}};

\pgfmathsetmacro{\r}{0.7391*\radius} 
\draw[colorEuclidean40](90-10*16:\r)--(0,0)--(90-10*17:\r) arc (90-10*17:90-10*16:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*33] at (90-5*33:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7391}$}};

\pgfmathsetmacro{\r}{0.8043*\radius} 
\draw[colorManhattan40](90-10*17:\r)--(0,0)--(90-10*18:\r) arc (90-10*18:90-10*17:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*35] at (90-5*35:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8043}$}};
% Recall Japanese

\pgfmathsetmacro{\r}{0.7912*\radius} 
\draw[colorChebychev40](90-10*18:\r)--(0,0)--(90-10*19:\r) arc (90-10*19:90-10*18:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*37+180] at (90-5*37:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7912}$}};

\pgfmathsetmacro{\r}{0.3736*\radius} 
\draw[colorEuclidean40](90-10*19:\r)--(0,0)--(90-10*20:\r) arc (90-10*20:90-10*19:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*39+180] at (90-5*39:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3736}$}};

\pgfmathsetmacro{\r}{0.8131*\radius} 
\draw[colorManhattan40](90-10*20:\r)--(0,0)--(90-10*21:\r) arc (90-10*21:90-10*20:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*41+180] at (90-5*41:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8131}$}};
% $F_1$ score Japanese

\pgfmathsetmacro{\r}{0.8044*\radius} 
\draw[colorChebychev40](90-10*21:\r)--(0,0)--(90-10*22:\r) arc (90-10*22:90-10*21:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*43+180] at (90-5*43:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8044}$}};

\pgfmathsetmacro{\r}{0.4963*\radius} 
\draw[colorEuclidean40](90-10*22:\r)--(0,0)--(90-10*23:\r) arc (90-10*23:90-10*22:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*45+180] at (90-5*45:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4963}$}};

\pgfmathsetmacro{\r}{0.8087*\radius} 
\draw[colorManhattan40](90-10*23:\r)--(0,0)--(90-10*24:\r) arc (90-10*24:90-10*23:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*47+180] at (90-5*47:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8087}$}};

% German

% AUC score German
\pgfmathsetmacro{\r}{0.4979*\radius} 
\draw[colorChebychev40](90-10*24:\r)--(0,0)--(90-10*25:\r) arc (90-10*25:90-10*24:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*49+180] at (90-5*49:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4979}$}};

\pgfmathsetmacro{\r}{0.5859*\radius} 
\draw[colorEuclidean40](90-10*25:\r)--(0,0)--(90-10*26:\r) arc (90-10*26:90-10*25:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*51+180] at (90-5*51:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.5859}$ }};


\pgfmathsetmacro{\r}{0.7696*\radius} 
\draw[colorManhattan40](90-10*26:\r)--(0,0)--(90-10*27:\r) arc (90-10*27:90-10*26:\r);
\pgfmathsetmacro{\r}{\radius + 3} 
\node[rotate=90-5*53+180] at (90-5*53:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7696}$}};

% Precision German
\pgfmathsetmacro{\r}{0.7237*\radius} 
\draw[colorChebychev40](90-10*27:\r)--(0,0)--(90-10*28:\r) arc (90-10*28:90-10*27:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*55+180] at (90-5*55:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7237}$}};


\pgfmathsetmacro{\r}{0.7568*\radius} 
\draw[colorEuclidean40](90-10*28:\r)--(0,0)--(90-10*29:\r) arc (90-10*29:90-10*28:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*57+180] at (90-5*57:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7568}$}};

\pgfmathsetmacro{\r}{0.8163*\radius} 
\draw[colorManhattan40](90-10*29:\r)--(0,0)--(90-10*30:\r) arc (90-10*30:90-10*29:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*59+180] at (90-5*59:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8163}$}};

% Recall score German

\pgfmathsetmacro{\r}{0.9958*\radius} 
\draw[colorChebychev40](90-10*30:\r)--(0,0)--(90-10*31:\r) arc (90-10*31:90-10*30:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*61+180] at (90-5*61:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.9958}$}};

\pgfmathsetmacro{\r}{0.7975*\radius} 
\draw[colorEuclidean40](90-10*31:\r)--(0,0)--(90-10*32:\r) arc (90-10*32:90-10*31:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*63+180] at (90-5*63:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7975}$}};

\pgfmathsetmacro{\r}{0.8264*\radius} 
\draw[colorManhattan40](90-10*32:\r)--(0,0)--(90-10*33:\r) arc (90-10*33:90-10*32:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*65+180] at (90-5*65:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8264}$}};


% $F_1$ score German

\pgfmathsetmacro{\r}{0.8382*\radius} 
\draw[colorChebychev40](90-10*33:\r)--(0,0)--(90-10*34:\r) arc (90-10*34:90-10*33:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*67+180] at (90-5*67:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8382}$}};

\pgfmathsetmacro{\r}{0.7766*\radius} 
\draw[colorEuclidean40](90-10*34:\r)--(0,0)--(90-10*35:\r) arc (90-10*35:90-10*34:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*69+180] at (90-5*69:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7766}$}};

\pgfmathsetmacro{\r}{0.8213*\radius} 
\draw[colorManhattan40](90-10*35:\r)--(0,0)--(90-10*36:\r) arc (90-10*36:90-10*35:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*71+180] at (90-5*71:\r) {\scalebox{1.175}[1.0]{\huge$\mathbf{0.8213}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 'Mercedes symbol' bold
\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorCamberra20] (0, 0) -- (90 - \a * 120 - \m * 120 : 1.6* \radius);
		}};
		
	
% Other bolds		

\foreach \m in {0, ..., 12}{
\draw[colorCamberra20] (0, 0) -- (90 - \m * 30 : 1.475* \radius);
};			
			
 Center
\draw[colorCamberra20, fill=white] (0,0) circle (0.2 * \radius);
\node at (0,0) {\Huge test data};
\draw[colorCamberra20, fill=white, yshift=\graphicshift cm] (0,0) circle (0.2 * \radius);
\node at (0,\graphicshift+0.5 cm){\Huge\textbf{Test Set}};
\node at (0,\graphicshift-0.5 cm){\Huge\textbf{}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Caption
\coordinate (rc) at (-20cm,-6cm \legendshift cm);
\foreach \m/\c in {GMM/colorChebychev,SVM/colorEuclidean,LR/colorManhattan} {
	\node[right of=rc, node distance=8cm, rectangle, draw=colorMainLines, fill=\c, minimum width=1.5cm, minimum height=0.825cm] (rc) {};
	\node[right of=rc, node distance=0.8cm, anchor=west] {\Huge \m};
}
			\end{tikzpicture}}
	\end{center}
	\caption{This figure compares the credit scoring results for Australia, Germany and Japan. We thank Francisco Antunes for providing us with the LaTeX template for creating the figure.}
\end{figure*}


==> figs/LaTeX_figs/confusion_matrices.tex <==
% %% 
% %% Copyright 2007, 2008, 2009 Elsevier Ltd
% %% 
% %% This file is part of the 'Elsarticle Bundle'.
% %% ---------------------------------------------
% %% 
% %% It may be distributed under the conditions of the LaTeX Project Public
% %% Author: Francisco Antunes

\begin{figure*}
	\begin{center}
	\resizebox{5in}{5in}{
			\begin{tikzpicture}
\pgfmathsetmacro{\radius}{20}
\pgfmathsetmacro{\graphicshift}{0}
\pgfmathsetmacro{\legendshift}{-30}

\definecolor{colorChebychev}{HTML}{55c968}

%\definecolor{colorEuclidean}{HTML}{800000}
\definecolor{colorEuclidean}{HTML}{DE4040}

%\definecolor{colorManhattan}{HTML}{FF0000}
\definecolor{colorManhattan}{HTML}{5872bf}

%\definecolor{colorCamberra}{HTML}{FF8000}
\definecolor{colorCamberra}{HTML}{2793DA}


\definecolor{colorMinkowsky}{HTML}{FFFF00}

\colorlet{colorLines}{gray!50!white}
\colorlet{colorMainLines}{gray}

\tikzset{colorEuclidean40/.style={fill=colorEuclidean,draw=black}}
\tikzset{colorManhattan40/.style={fill=colorManhattan,draw=black}}
\tikzset{colorCamberra40/.style={fill=colorCamberra,draw=black}}
\tikzset{colorChebychev40/.style={fill=colorChebychev,draw=black}}
\tikzset{colorMinkowsky40/.style={fill=colorMinkowsky,draw=black}}

\tikzset{colorEuclidean20/.style={draw=black,line width=0.1cm}}
\tikzset{colorManhattan20/.style={draw=black,line width=0.1cm}}
\tikzset{colorCamberra20/.style= {draw=black,line width=0.1cm}}
\tikzset{colorChebychev20/.style={draw=black,line width=0.1cm}}
\tikzset{colorMinkowsky20/.style={draw=black,line width=0.1cm}}

\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorCamberra40] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		}};
	
% 10º arches		
\foreach \a in {0, ..., 5} {
	\foreach \m in {0, ..., 16} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 10: 1.3* \radius);
		}};		
	
\foreach \a in {0, ..., 2} {
	\foreach \m in {0, ..., 3} {
		\draw[colorMainLines] (0, 0) -- (90 - \a * 120 - \m * 40 : 1.3* \radius);
		};
\draw[colorMainLines] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
	\draw[colorMainLines, yshift=\graphicshift cm] (0, 0) -- (90 - \a * 120 : 1.475 * \radius);
};

% Concentric Circles


\foreach \p in {1.0, 1.475, 1.3, 1.6} %{0.5,0.1,0.15,0.2,0.25,0.3,0.35,0.4,0.45,0.5,0.55,0.6,0.65,0.7,0.75,0.8,0.85,0.9, 0.95,1.0, 1.475, 1.3, 1.6}
{
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorLines] (0,0) circle (\r);
	\draw[colorLines, yshift=\graphicshift cm] (0,0) circle (\r);	
};

\foreach \p in {1} {
	\pgfmathsetmacro{\r}{\p * \radius}
	\draw[colorCamberra20] (0,0) circle (\r);
	\draw[colorCamberra20, yshift=\graphicshift cm] (0,0) circle (\r);	
};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metrics - False Negative Header
\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (75:\r) {\Huge{\textbf{Germany}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (45:\r) {\Huge{\textbf{Australia}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-75] at (15:\r) {\Huge{\textbf{Japan}}};



\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=-45] at (45:\r) {\Huge{\textbf{False Negative}}};

% Metrics - True Negative Header


\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-105] at (-15:\r) {\Huge{\textbf{Germany}}};


\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+25+40+40+40+40+40:\r) {\Huge{\textbf{Australia}}};


\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+25+10+40+40+40+40:\r) {\Huge{\textbf{Japan}}};


\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=45] at (30-120+45:\r) {\Huge{\textbf{True Negative}}};

% Metrics - False positive Header


\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-15] at (90+20-15+40+40+40+40:\r) {\Huge{\textbf{Germany}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=-45] at (90+20-15+40+40+40+40-30:\r) {\Huge{\textbf{Australia}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=105] at (90+15+30+30+30:\r) {\Huge{\textbf{Japan}}};

% Metrics - True positive Header



\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=15] at (90+15:\r) {\Huge{\textbf{Japan}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=45] at (90+15+30:\r) {\Huge{\textbf{Australia}}};

\pgfmathsetmacro{\r}{\radius + 7.5}
\node[rotate=75] at (90+15+30+30:\r) {\Huge{\textbf{Germany}}};




\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=-45] at (30-120-45:\r) {\Huge{\textbf{False Positive}}};



\pgfmathsetmacro{\r}{\radius + 10.5}
\node[rotate=45] at (15-120*2:\r) {\Huge{\textbf{True Positive}}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% False Negative
% AUC score False Negative
\pgfmathsetmacro{\r}{92/241*\radius} 
\draw[colorChebychev40](90:\r)--(0,0)--(90-10*1:\r) arc (90-10*1:90:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*1] at (90-5*1:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{92}$}};

\pgfmathsetmacro{\r}{62/241*\radius} 
\draw[colorEuclidean40](90-10*1:\r)--(0,0)--(90-10*2:\r) arc (90-10*2:90-10*1:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*3] at (90-5*3:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{62}$}};

\pgfmathsetmacro{\r}{45/241*\radius} 
\draw[colorManhattan40](90-10*2:\r)--(0,0)--(90-10*3:\r) arc (90-10*3:90-10*2:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*5] at (90-5*5:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{45}$}};

% Precision False Negative

\pgfmathsetmacro{\r}{13/119*\radius} 
\draw[colorChebychev40](90-10*3:\r)--(0,0)--(90-10*4:\r) arc (90-10*4:90-10*3:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*7] at (90-5*7:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{13}$}};

\pgfmathsetmacro{\r}{10/119*\radius} %dois
\draw[colorEuclidean40](90-10*4:\r)--(0,0)--(90-10*5:\r) arc (90-10*5:90-10*4:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*9] at (90-5*9:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{10}$}};

\pgfmathsetmacro{\r}{13/119*\radius} %dois
\draw[colorManhattan40](90-10*5:\r)--(0,0)--(90-10*6:\r) arc (90-10*6:90-10*5:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*11] at (90-5*11:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{13}$}};

% Recall False Negative


\pgfmathsetmacro{\r}{0.6732*\radius} %dois
\draw[colorChebychev40](90-10*6:\r)--(0,0)--(90-10*7:\r) arc (90-10*7:90-10*6:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*13] at (90-5*13:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.6732}$}};

\pgfmathsetmacro{\r}{0.3267*\radius} %dois
\draw[colorEuclidean40](90-10*7:\r)--(0,0)--(90-10*8:\r) arc (90-10*8:90-10*7:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*15] at (90-5*15:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3267}$}};

\pgfmathsetmacro{\r}{0.7128*\radius} %dois
\draw[colorManhattan40](90-10*8:\r)--(0,0)--(90-10*9:\r) arc (90-10*9:90-10*8:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*17] at (90-5*17:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7128}$}};
% $F_1$ score False Negative
\pgfmathsetmacro{\r}{0.7472*\radius} 
\draw[colorChebychev40](90-10*9:\r)--(0,0)--(90-10*10:\r) arc (90-10*10:90-10*9:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*19] at (90-5*19:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7472}$}};

\pgfmathsetmacro{\r}{0.4583*\radius} 
\draw[colorEuclidean40](90-10*10:\r)--(0,0)--(90-10*11:\r) arc (90-10*11:90-10*10:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*21] at (90-5*21:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4583}$}};

\pgfmathsetmacro{\r}{0.7741*\radius} 
\draw[colorManhattan40](90-10*11:\r)--(0,0)--(90-10*12:\r) arc (90-10*12:90-10*11:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*23] at (90-5*23:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7741}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sampling True Negative

% AUC score True Negative

\pgfmathsetmacro{\r}{0.8340*\radius} 
\draw[colorChebychev40](90-10*12:\r)--(0,0)--(90-10*13:\r) arc (90-10*13:90-10*12:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*25] at (90-5*25:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8340}$}};

\pgfmathsetmacro{\r}{0.7321*\radius} 
\draw[colorEuclidean40](90-10*13:\r)--(0,0)--(90-10*14:\r) arc (90-10*14:90-10*13:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*27] at (90-5*27:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7321}$}};

\pgfmathsetmacro{\r}{0.8692*\radius} 
\draw[colorManhattan40](90-10*14:\r)--(0,0)--(90-10*15:\r) arc (90-10*15:90-10*14:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*29] at (90-5*29:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8692}$}};
% Precision True Negative

\pgfmathsetmacro{\r}{0.8181*\radius} 
\draw[colorChebychev40](90-10*15:\r)--(0,0)--(90-10*16:\r) arc (90-10*16:90-10*15:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*31] at (90-5*31:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8181}$}};

\pgfmathsetmacro{\r}{0.7391*\radius} 
\draw[colorEuclidean40](90-10*16:\r)--(0,0)--(90-10*17:\r) arc (90-10*17:90-10*16:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*33] at (90-5*33:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7391}$}};

\pgfmathsetmacro{\r}{0.8043*\radius} 
\draw[colorManhattan40](90-10*17:\r)--(0,0)--(90-10*18:\r) arc (90-10*18:90-10*17:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*35] at (90-5*35:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8043}$}};
% Recall True Negative

\pgfmathsetmacro{\r}{0.7912*\radius} 
\draw[colorChebychev40](90-10*18:\r)--(0,0)--(90-10*19:\r) arc (90-10*19:90-10*18:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*37+180] at (90-5*37:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7912}$}};

\pgfmathsetmacro{\r}{0.3736*\radius} 
\draw[colorEuclidean40](90-10*19:\r)--(0,0)--(90-10*20:\r) arc (90-10*20:90-10*19:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*39+180] at (90-5*39:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.3736}$}};

\pgfmathsetmacro{\r}{0.8131*\radius} 
\draw[colorManhattan40](90-10*20:\r)--(0,0)--(90-10*21:\r) arc (90-10*21:90-10*20:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*41+180] at (90-5*41:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8131}$}};
% $F_1$ score True Negative

\pgfmathsetmacro{\r}{0.8044*\radius} 
\draw[colorChebychev40](90-10*21:\r)--(0,0)--(90-10*22:\r) arc (90-10*22:90-10*21:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*43+180] at (90-5*43:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8044}$}};

\pgfmathsetmacro{\r}{0.4963*\radius} 
\draw[colorEuclidean40](90-10*22:\r)--(0,0)--(90-10*23:\r) arc (90-10*23:90-10*22:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*45+180] at (90-5*45:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4963}$}};

\pgfmathsetmacro{\r}{0.8087*\radius} 
\draw[colorManhattan40](90-10*23:\r)--(0,0)--(90-10*24:\r) arc (90-10*24:90-10*23:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*47+180] at (90-5*47:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8087}$}};

% German

% AUC score German
\pgfmathsetmacro{\r}{0.4979*\radius} 
\draw[colorChebychev40](90-10*24:\r)--(0,0)--(90-10*25:\r) arc (90-10*25:90-10*24:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*49+180] at (90-5*49:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.4979}$}};

\pgfmathsetmacro{\r}{0.5859*\radius} 
\draw[colorEuclidean40](90-10*25:\r)--(0,0)--(90-10*26:\r) arc (90-10*26:90-10*25:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*51+180] at (90-5*51:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.5859}$ }};


\pgfmathsetmacro{\r}{0.7696*\radius} 
\draw[colorManhattan40](90-10*26:\r)--(0,0)--(90-10*27:\r) arc (90-10*27:90-10*26:\r);
\pgfmathsetmacro{\r}{\radius + 3} 
\node[rotate=90-5*53+180] at (90-5*53:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7696}$}};

% Precision German
\pgfmathsetmacro{\r}{1.7237/2*\radius} 
\draw[colorChebychev40](90-10*27:\r)--(0,0)--(90-10*28:\r) arc (90-10*28:90-10*27:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*55+180] at (90-5*55:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7237}$}};


\pgfmathsetmacro{\r}{0.7568*\radius} 
\draw[colorEuclidean40](90-10*28:\r)--(0,0)--(90-10*29:\r) arc (90-10*29:90-10*28:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*57+180] at (90-5*57:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7568}$}};

\pgfmathsetmacro{\r}{0.8163*\radius} 
\draw[colorManhattan40](90-10*29:\r)--(0,0)--(90-10*30:\r) arc (90-10*30:90-10*29:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*59+180] at (90-5*59:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8163}$}};

% Recall score German

\pgfmathsetmacro{\r}{0.9958*\radius} 
\draw[colorChebychev40](90-10*30:\r)--(0,0)--(90-10*31:\r) arc (90-10*31:90-10*30:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*61+180] at (90-5*61:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.9958}$}};

\pgfmathsetmacro{\r}{0.7975*\radius} 
\draw[colorEuclidean40](90-10*31:\r)--(0,0)--(90-10*32:\r) arc (90-10*32:90-10*31:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*63+180] at (90-5*63:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7975}$}};

\pgfmathsetmacro{\r}{0.8264*\radius} 
\draw[colorManhattan40](90-10*32:\r)--(0,0)--(90-10*33:\r) arc (90-10*33:90-10*32:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*65+180] at (90-5*65:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8264}$}};


% $F_1$ score German

\pgfmathsetmacro{\r}{0.8382*\radius} 
\draw[colorChebychev40](90-10*33:\r)--(0,0)--(90-10*34:\r) arc (90-10*34:90-10*33:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*67+180] at (90-5*67:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.8382}$}};

\pgfmathsetmacro{\r}{0.7766*\radius} 
\draw[colorEuclidean40](90-10*34:\r)--(0,0)--(90-10*35:\r) arc (90-10*35:90-10*34:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*69+180] at (90-5*69:\r) {\scalebox{1.175}[1.0]{\huge $\mathbf{0.7766}$}};

\pgfmathsetmacro{\r}{0.8213*\radius} 
\draw[colorManhattan40](90-10*35:\r)--(0,0)--(90-10*36:\r) arc (90-10*36:90-10*35:\r);
\pgfmathsetmacro{\r}{\radius + 3}
\node[rotate=90-5*71+180] at (90-5*71:\r) {\scalebox{1.175}[1.0]{\huge$\mathbf{0.8213}$}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 'Mercedes symbol' bold
% \foreach \a in {0, ..., 2} {
% 	\foreach \m in {0, ..., 3} {
% 		\draw[colorCamberra20] (0, 0) -- (90 - \a * 120 - \m * 120 : 1.6* \radius);
% 		}};

\foreach \a in {0, ..., 3} {
		\draw[colorCamberra20] (0, 0) -- (90 * \a : 1.6* \radius);
		};	


% Other bolds		
% \foreach \a in {0, ..., 3} {
% 	\foreach \m in {0, ..., 3} {
% 		\draw[colorCamberra20] (0, 0) -- (90 - \a * 80 - \m * 30 : 1.475* \radius);
% 		}};
			
\foreach \m in {0, ..., 12}{
\draw[colorCamberra20] (0, 0) -- (90 - \m * 30 : 1.475* \radius);
};			
			
 Center
% \draw[colorCamberra20, fill=white] (0,0) circle (0.05 * \radius);
\node at (0,0) {\Huge test data};
\draw[colorCamberra20, fill=white, yshift=\graphicshift cm] (0,0) circle (0.1 * \radius);
\node at (0,\graphicshift+0.5 cm){\Huge\textbf{Test }};
\node at (0,\graphicshift-0.5 cm){\Huge\textbf{Set}};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Caption
\coordinate (rc) at (-20cm,-6cm \legendshift cm);
\foreach \m/\c in {GMM/colorChebychev,SVM/colorEuclidean,LR/colorManhattan} {
	\node[right of=rc, node distance=8cm, rectangle, draw=colorMainLines, fill=\c, minimum width=1.5cm, minimum height=0.825cm] (rc) {};
	\node[right of=rc, node distance=0.8cm, anchor=west] {\Huge \m};
}
			\end{tikzpicture}}
	\end{center}
	\caption{This figure will sh}
\end{figure*}


==> tabs/tab_Australia_cluster.tex <==
\begin{table}
\centering
\caption{Clusters' features in Australian Data set}
\begin{tabular}{lcccccccccc}
\toprule
          & \textbf{Cluster} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
    \midrule
    \multirow{5}[2]{*}{\textbf{Train}} & \textbf{Goods} & 40    & 2     & 2     & 4     & 10    & 19    & 2     & 7     & 120 \\
          & \textbf{Bads} & 118   & 0     & 0     & 0     & 4     & 114   & 0     & 7     & 11 \\
          & \textbf{ratio} & 0.34  & --    & --    & --    & 2.50  & 0.17  & --    & 1.00  & 10.91 \\
          & \textbf{probability} & 0.25  & 1.00  & 1.00  & 1.00  & 0.71  & 0.14  & 1.00  & 0.50  & 0.92 \\
          & \textbf{weight} & \multicolumn{1}{r}{\textcolor[rgb]{ .129,  .129,  .129}{0.34}} & 0.00  & 0.00  & 0.01  & 0.03  & 0.29  & 0.00  & 0.03  & 0.28 \\
    \midrule
    \multirow{3}[1]{*}{\textbf{Test}} & \textbf{Goods} & 20    & 0     & 0     & 0     & 2     & 13    & 0     & 0     & 66 \\
          & \textbf{Bads} & 54    & 0     & 0     & 0     & 1     & 62    & 0     & 0     & 12 \\
          & \textbf{ratio} & 0.37  & --    & --    & --    & 2.00  & 0.21  & --    & --    & 5.50 \\
    \bottomrule
\end{tabular}%
\label{tab_Australian_clusters}%
\end{table}%


==> tabs/tab_German_clusters.tex <==
\begin{table}
\centering
\caption{Clusters' features in German Data set}
\begin{tabular}{lcccccccccc}
\toprule
          & \textbf{Cluster} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
    \midrule
    \multirow{5}[2]{*}{\textbf{Train}} & \textbf{Goods} & 31    & 20    & 2     & 2     & 76    & 9     & 20    & 31    & 267 \\
          & \textbf{Bads} & 20    & 26    & 202   & 9     & 26    & 18    & 16    & 23    & 118 \\
          & \textbf{ratio} & 1.55  & 0.77  & 0.01  & 0.22  & 2.92  & 0.50  & 1.25  & 1.35  & 2.26 \\
          & \textbf{probability} & 0.61  & 0.43  & 0.01  & 0.18  & 0.75  & 0.33  & 0.56  & 0.57  & 0.69 \\
          & \textbf{weight} & 0.06  & 0.05  & 0.22  & 0.01  & 0.11  & 0.03  & 0.04  & 0.06  & 0.42 \\
    \cmidrule{2-11}
    \multirow{3}[1]{*}{\textbf{Test}} & \textbf{Goods} & 2     & 0     & 1     & 0     & 72    & 0     & 0     & 6     & 161 \\
          & \textbf{Bads} & 1     & 0     & 0     & 0     & 39    & 0     & 0     & 0     & 52 \\
          & \textbf{ratio} & 2.00  & --    & --    & --    & 1.85  & --    & --    & --    & 3.10 \\
    \bottomrule
\end{tabular}%
\label{tab_germans_cluster}%
\end{table}%


==> tabs/tab_Japan_cluster.tex <==
\begin{table}
\centering
\caption{Clusters' features in Japan Data set}
\begin{tabular}{lcccccccccc}
\toprule
          & \textbf{Cluster} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
    \midrule
    \multirow{5}[2]{*}{\textbf{Train}} & \textbf{Goods} & 11    & 1     & 147   & 3     & 1     & 18    & 7     & 2     & 16 \\
          & \textbf{Bads} & 40    & 0     & 24    & 0     & 0     & 42    & 0     & 0     & 128 \\
          & \textbf{ratio} & 0.28  & --    & 6.13  & --    & --    & 0.43  & --    & --    & 0.13 \\
          & \textbf{probability} & 0.21  & 1.00  & 0.86  & 1.00  & 1.00  & 0.30  & 1.00  & 1.00  & 0.11 \\
          & \textbf{weight} & 0.12  & 0.00  & 0.39  & 0.01  & 0.00  & 0.14  & 0.02  & 0.00  & 0.33 \\
    \midrule
    \multirow{3}[1]{*}{\textbf{Test}} & \textbf{Goods} & 3     & 0     & 72    & 0     & 0     & 7     & 0     & 0     & 9 \\
          & \textbf{Bads} & 24    & 0     & 16    & 0     & 0     & 18    & 0     & 0     & 72 \\
          & \textbf{ratio} & 0.13  & --    & 4.50  & --    & --    & 0.39  & --    & --    & 0.13 \\
    \bottomrule
\end{tabular}%
\label{tab_japan_clusters}%
\end{table}%


==> tabs/tab_accuracy.tex <==
\begin{table}
  \centering
  \caption{Comparison of our model's accuracy to SVM and LR}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}

    \toprule
          & \multicolumn{2}{c}{Germany} & \multicolumn{2}{c}{Japan} & \multicolumn{2}{c}{Australia} \\
          & \multicolumn{1}{c}{train} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{train} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{train} & \multicolumn{1}{c}{test} \\
    \midrule
    GMM & 74.23\% & 72.15\% & 84.31\% & 84.16\% & 82.39\% & 80.00\% \\
    SVM   & 54.80\% & 66.76\% & 65.68\% & 68.77\% & 66.52\% & 66.08\% \\
    LR    & 82.31\% & 73.95\% & 82.50\% & 84.10\% & 84.56\% & 81.73\% \\
    \bottomrule
    \end{tabular}%
}
    \label{tab_accuracies}%
    
    
% \vspace{1ex}
%      {\raggedright Note: looking at the results for the German and Australian data sets, GMM performs far better than SVM in both train and test sets and its performance compared with LR is competitive. The GMM also avoids over-fitting on the German data set, in contrary to LR. For the Japanese data set, GMM is superior to both benchmarks. 
%      \par}  
\end{table}%


==> tabs/tab_clusters2.tex <==
% \multirow{8}[3]{*}{\begin{sideways}German Data\end{sideways}}
% \multirow{8}[3]{*}{\begin{sideways}Japanese Data\end{sideways}}
% \multirow{8}[3]{*}{\begin{sideways}Australian Data\end{sideways}}

\begin{table}
\centering
\caption{Clusters' features in the German, Japan, and Australian Data sets}
\begin{tabular}{llccccccccc}
& \multirow{}{c}{Clusters}
      &       &  & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} \\
 & \multirow{5}[1]{*}{\textbf{Train}} & \textbf{Good applicants} & 31    & 20    & 2     & 2     & 76    & 9     & 20    & 31    & 267 \\
      &       & \textbf{Bad applicants} & 20    & 26    & 202   & 9     & 26    & 18    & 16    & 23    & 118 \\
      &       & \textbf{Ratio} & 1.55  & 0.77  & 0.01  & 0.22  & 2.92  & 0.50  & 1.25  & 1.35  & 2.26 \\
      &       & \textbf{Probability} & 0.61  & 0.43  & 0.01  & 0.18  & 0.75  & 0.33  & 0.56  & 0.57  & 0.69 \\
      &       & \textbf{Weight} & 0.06  & 0.05  & 0.22  & 0.01  & 0.11  & 0.03  & 0.04  & 0.06  & 0.42 \\
\cmidrule{4-12}      & \multirow{3}[2]{*}{\textbf{Test}} & \textbf{Good applicants} & 2     & 0     & 1     & 0     & 72    & 0     & 0     & 6     & 161 \\
      &       & \textbf{Bad  applicants} & 1     & 0     & 0     & 0     & 39    & 0     & 0     & 0     & 52 \\
      &       & \textbf{Ratio} & 2.00  & --    & --    & --    & 1.85  & --    & --    & --    & 3.10 \\
\midrule
& \multirow{5}[2]{*}{\textbf{Train}} & \textbf{Good applicants} & 11    & 1     & 147   & 3     & 1     & 18    & 7     & 2     & 16 \\
      &       & \textbf{Bad applicants} & 40    & 0     & 24    & 0     & 0     & 42    & 0     & 0     & 128 \\
      &       & \textbf{Ratio} & 0.28  & --    & 6.13  & --    & --    & 0.43  & --    & --    & 0.13 \\
      &       & \textbf{Probability} & 0.21  & 1.00  & 0.86  & 1.00  & 1.00  & 0.30  & 1.00  & 1.00  & 0.11 \\
      &       & \textbf{Weight} & 0.12  & 0.00  & 0.39  & 0.01  & 0.00  & 0.14  & 0.02  & 0.00  & 0.33 \\
\cmidrule{4-12}      & \multirow{3}[1]{*}{\textbf{Test}} & \textbf{Good applicants} & 3     & 0     & 72    & 0     & 0     & 7     & 0     & 0     & 9 \\
      &       & \textbf{Bad  applicants} & 24    & 0     & 16    & 0     & 0     & 18    & 0     & 0     & 72 \\
      &       & \textbf{Ratio} & 0.13  & --    & 4.50  & --    & --    & 0.39  & --    & --    & 0.13 \\
& \multirow{5}[1]{*}{\textbf{Train}} & \textbf{Good applicants} & 40    & 2     & 2     & 4     & 10    & 19    & 2     & 7     & 120 \\
      &       & \textbf{Bad applicants} & 118   & 0     & 0     & 0     & 4     & 114   & 0     & 7     & 11 \\
      &       & \textbf{Ratio} & 0.34  & --    & --    & --    & 2.50  & 0.17  & --    & 1.00  & 10.91 \\
      &       & \textbf{Probability} & 0.25  & 1.00  & 1.00  & 1.00  & 0.71  & 0.14  & 1.00  & 0.50  & 0.92 \\
      &       & \textbf{Weight} & 0.34  & 0.00  & 0.00  & 0.01  & 0.03  & 0.29  & 0.00  & 0.03  & 0.28 \\
\cmidrule{4-12}      & \multirow{3}[2]{*}{\textbf{Test}} & \textbf{Good applicants} & 20    & 0     & 0     & 0     & 2     & 13    & 0     & 0     & 66 \\
      &       & \textbf{Bad  applicants} & 54    & 0     & 0     & 0     & 1     & 62    & 0     & 0     & 12 \\
      &       & \textbf{Ratio} & 0.37  & --    & --    & --    & 2.00  & 0.21  & --    & --    & 5.50 \\
\bottomrule
\end{tabular}%
\label{tab_clusters}%
\vspace{1ex}
     {\raggedright Note: \color{red}  This table presents back-testing results of various VaR methods, including Uncertain EVT, EVT GARCH, EGARCH, CaviaR asymmetric, Monte Carlo Simulation, Historical Simulation and Variance-Covariance using unconditional coverage test (Kupiec) and conditional coverage test (Christoffersen). Unconditional coverage test only cares about the number of violations not to exceed a predetermined confidence interval but conditional coverage test also considers successive violations. In this table, LR UC and LR CC refer to likelihood ratio unconditional and conditional coverage tests, respectively. As per the results of these coverage tests, NR stands for not rejected and R stands for rejected results. Two of the most successful methods based on the results on global indices S\&P500, FTSE 100, Dow Jones, Nikkei, BVSP and Mervel are the Undertain EVT and GARCH methods. 
     \par}
\end{table}%


==> tabs/tab_prob_loss_rnd.tex <==
\begin{table}[width=2.0\linewidth,cols=8, pos = t]
\centering
\caption{Actual loss and predicted loss for different models and their errors with a random amount of loan with a mean of $1000$\$}
\begin{tabular}{lccccccc}
    \toprule
          & \multicolumn{1}{l}{actual loss} & \multicolumn{1}{l}{predicted loss} & \multicolumn{1}{l}{predicted loss } & \multicolumn{1}{l}{predicted loss} & \multicolumn{1}{l}{error} & \multicolumn{1}{l}{error} & \multicolumn{1}{l}{error} \\
          &       & \multicolumn{1}{l}{GMM} & \multicolumn{1}{l}{SVM} & \multicolumn{1}{l}{LR} & \multicolumn{1}{l}{ GMM} & \multicolumn{1}{l}{SVM} & \multicolumn{1}{l}{LR} \\
    \midrule
    Train &       &       &       &       &       &       &  \\
    Germany & 228995 & 229128 & 228513 & 226541 & 0.06  & 0.27  & 0.86 \\
    Japan & 117515 & 117134 & 115816 & 113235 & 0.32  & 1.13  & 2.23 \\
    Australia & 128192 & 127575 & 126342 & 130715 & 0.48  & 0.97  & 3.46 \\
    \midrule
    Test  &       &       &       &       &       &       &  \\
    Germany & 46407 & 49193 & 83621 & 55570 & 6.00  & 69.99 & 33.55 \\
    Japan & 64335 & 60962 & 57285 & 57115 & 5.24  & 6.03  & 0.30 \\
    Australia & 63694 & 62457 & 62243 & 65825 & 1.94  & 0.34  & 5.75 \\
    \bottomrule
\end{tabular}%
\label{tab_prob_loss_rnd}%
\end{table}
